BagPack: A general framework to represent semantic relations

We introduce a way to represent word pairs instantiating arbitrary semantic relations that keeps track of the contexts in which the words in the pair occur both together and independently. The resulting features are of sufficient generality to allow us, with the help of a standard supervised machine learning algorithm, to tackle a variety of unrelated semantic tasks with good results and almost no task-specific tailoring.

==> conclusion.tex <==
\section{Conclusions}
\label{sec:conclusions}

We presented a general way to build a vector-based space to represent
the semantic relations between word pairs and showed how that
representation can be used to solve various tasks involving semantic
similarity. For SAT and TOEFL, we obtained reasonable performances
comparable to the state of the art. For the estimation of selective
preference judgments about verb-noun pairs, we achieved state of the
art performance. Perhaps more importantly, our representation format
allows us to provide meaningful estimates even when the verb and noun
are not observed co-occurring in the corpus -- which is an obvious
advantage over the models which rely on sytagmatic contexts alone and
cannot provide estimates for word pairs that are not seen directly
co-occurring. We also obtained very promising results for the
automated augmentation of ConceptNet.

The generality of the proposed method is also reflected in the fact
that we built a single feature space based on frequent basis terms and
used the same features for all pairs coming from different tasks. The
use of the same feature set for all pairs makes it possible to build a
single database of word-pair vectors. For example, we were able to
re-use the vectors constructed for SAT pairs as a validation set in
the ConceptNet task. Furthermore, the results reported here are
obtained for the same machine learning model (SVM) without any
parameter tweaking, which renders them very strict lower bounds.

Another contribution is that the proposed method provides a way
to represent the relations between words even if they are not observed
co-occurring in the corpus. Employing a larger corpus can be an
alternative solution for some cases but this is not always possible
and some tasks, like estimating selectional preference judgments,
inherently call for a method that does not exclusively depends on
paired co-occurrence observations.

Finally, we introduced ConceptNet, a common-sense semantic network, to
the corpus-based semantics community, both as a new challenge and as a
repository we can benefit from.

In future work, one of the most pressing issue we want to explore is
how to better exploit the information in the single occurrence
vectors: currently, we do not make any use of the \emph{overlap}
between $\mathbf{v_{1}}$ and $\mathbf{v_{2}}$. In this way, we are
missing the classic intuition that taxonomically similar words tend to
occur in similar contexts, and it is thus not surprising that
$\mathbf{v_{1}v_{2}}$ flunks the TOEFL. We are currently looking at
ways to augment our concatenated vector with ``meta-information''
about vector overlap.


==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Co-occurrence statistics extracted from corpora lead to good
performance on a wide range of tasks that involve the identification
of the semantic relation between two words or concepts
\cite{Sahlgren:2006,Turney:2006}. However, the difficulty of such
tasks and the fact that they are apparently unrelated has led to the
development of largely \emph{ad-hoc} solutions, tuned to specific
challenges. For many practical applications, this is a drawback: Given
the large number of semantic relations that might be relevant to one
or the other task, we need a multi-purpose approach that, given an
appropriate representation and training examples instantiating an
arbitrary target relation, can automatically mine new pairs
characterized by the same relation. Building on a recent proposal in
this direction by \newcite{Turney:2008}, we propose a generic method
of this sort, and we test it on a set of unrelated tasks, reporting
good performance across the board with very little task-specific
tweaking.

There has been much previous work on corpus-based models to extract
broad classes of related words. The literature on word space models
\cite{Sahlgren:2006} has focused on taxonomic similarity (synonyms,
antonyms, co-hyponyms\ldots) and general association (e.g., finding
topically related words), exploiting the idea that taxonomically or
associated words will tend to occur in similar contexts, and thus
share a vector of co-occurring words. The literature on relational
similarity, on the other hand, has focused on \emph{pairs} of words,
devising various methods to compare how similar the contexts in which
target pairs appear are to the contexts of other pairs that
instantiate a relation of interest
\cite{Turney:2006,Pantel:Pennacchiotti:2006}. Beyond these domains,
purely corpus-based methods play an increasingly important role in
modeling constraints on composition of words, in particular verbal
selectional preferences -- finding out that, say, children are more
likely to eat than apples, whereas the latter are more likely to be
eaten \cite{Erk:2007,Pado:etal:2007}. Tasks of this sort differ from
relation extraction in that we need to capture \emph{productive}
patterns: we want to find out that shabu shabu (a Japanese meat dish)
is eaten whereas ink is not, even if in our corpus neither noun is
attested in proximity to forms of the verb \emph{to eat}. 

\newcite{Turney:2008} is the first, to the best of our knowledge, to
raise the issue of a unified approach. In particular, he treats
synonymy and association as special cases of relational similarity: in
the same way in which we might be able to tell that hands and arms are
in a part-of relation by comparing the contexts in which they co-occur
to the contexts of known part-of pairs, we can guess that cars and
automobiles are synonyms by comparing the contexts in which they
co-occur to the contexts linking known synonym pairs.

Here, we build on Turney's work, adding two main methodological
innovations that allow us further generalization. First, merging
classic approaches to taxonomic and relational similarity, we
represent concept pairs by a vector that concatenates information
about the contexts in which the two words occur independently, and the
contexts in which they co-occur (Mirkin et al.~2006 also integrate
information from the lexical patterns in which two words co-occur and
similarity of the contexts in which each word occurs on its own, to
improve performance in lexical entailment acquisition). Second, we
represent contexts as bag of words and bigrams, rather than strings of
words (``patterns'') of arbitrary length: we leave it to the machine
learning algorithm to zero in on the most interesting words/bigrams.

Thanks to the concatenated vector, we can tackle tasks in which the
two words are not expected to co-occur even in very large corpora
(such as selectional preference). Concatenation, together with
unigram/bigram representation of context, allows us to scale down the
approach to smaller training corpora (Turney used a corpus of more
than 50 billion words), since we do not need to see the words directly
co-occurring, and the unigram/bigram dimensions of the vectors are
less sparse than dimensions based on longer strings of words. We show
that our method produces reasonable results also on a corpus of 2
billion words, with many unseen pairs. Moreover, our bigram and
unigram representation is general enough that we do not need to
extract separate statistics nor perform \emph{ad-hoc} feature selection for
each task: we build the co-occurrence matrix once, and use the same
matrix in all experiments. The bag-of-words assumption also makes for
faster and more compact model building, since the number of features
we extract from a context is linear in the number of words in the
context, whereas it is exponential for Turney. On the other hand, our
method is currently lagging behind Turney's in terms of performance,
suggesting that at least some task-specific tuning will be necessary.

Following Turney, we focus on devising a suitably general featural
representation, and we see the specific machine learning algorithm
employed to perform the various tasks as a parameter. Here, we use
Support Vector Machines since they are a particularly effective
general-purpose method. In terms of empirical evaluation of the model,
besides experimenting with the ``classic'' SAT and TOEFL datasets, we
show how our algorithm can tackle the selectional preference task
proposed in \newcite{Pado:2007} -- a regression task -- and we
introduce to the corpus-based semantics community a challenge from the
ConceptNet repository of common-sense knowledge (extending such
repository by automated means is the original motivation of our
project).

In the next section, we will present our proposed method along with
the corpora and model parameter choices used in the implementation. In
Section~\ref{sec:tasks}, we describe the tasks that we use to evaluate
the model. Results are reported in Section \ref{sec:results} and we
conclude in Section~\ref{sec:conclusions}, with a brief overview of
the contributions of this paper.

